Publicly Verifiable Deletion from Minimal Assumptions

We present a general compiler to add the publicly verifiable deletion property for various cryptographic primitives including public key encryption, attribute-based encryption, and quantum fully homomorphic encryption. Our compiler only uses one-way functions, or more generally hard quantum planted problems for NP, which are implied by one-way functions. It relies on minimal assumptions and enables us to add the publicly verifiable deletion property with no additional assumption for the above primitives. Previously, such a compiler needs additional assumptions such as injective trapdoor one-way functions or pseudorandom group actions [Bartusek-Khurana-Poremba, ePrint:2023/370]. Technically, we upgrade an existing compiler for privately verifiable deletion [Bartusek-Khurana, ePrint:2022/1178] to achieve publicly verifiable deletion by using digital signatures.

==> preamble_newtheorem.tex <==
\newtheorem{theorem}{Theorem} 
\newtheorem{lemma}{Lemma} 
\newtheorem{claim}{Claim}  
\newtheorem{proposition}{Proposition} 
\newtheorem{definition}{Definition}  
\newtheorem{fact}{Fact}  
\newtheorem{remark}{Remark}  
%\newtheorem{proof}{Proof}  % Already defined by ``amsthm" package. Only include it when ``amsthm" is not used.
\newtheorem{corollary}{Corollary} 
